Self-Aware Personalized Federated Learning

In the context of personalized federated learning (FL), the critical challenge is to balance local model improvement and global model tuning when the personal and global objectives may not be exactly aligned. Inspired by Bayesian hierarchical models, we develop a self-aware personalized FL method where each client can automatically balance the training of its local personal model and the global model that implicitly contributes to other clients' training. Such a balance is derived from the inter-client and intra-client uncertainty quantification. A larger inter-client variation implies more personalization is needed. Correspondingly, our method uses uncertainty-driven local training steps and aggregation rule instead of conventional local fine-tuning and sample size-based aggregation. With experimental studies on synthetic data, Amazon Alexa audio data, and public datasets such as MNIST, FEMNIST, CIFAR10, and Sent140, we show that our proposed method can achieve significantly improved personalization performance compared with the existing counterparts.

==> addition.tex <==
\section{Summary of Notations}

Some frequently used notations are summarized in Table~\ref{tab_notation}.

\begin{table*}[tb]
\caption{Frequently used notations} \label{tab_notation}
\begin{tabular}{lll}
\hline
Notation            & Meaning                                                                                    &  \\ \hline
$M$                 & number of clients                                                                          &  \\
$\vD_m$             & variance of client $m$'s estimated parameters, or the ``intra-client uncertainty'' in general                                              &  \\
$\vT$               & variance of different clients' underlying parameters, or the ``inter-client uncertainty'' in general                                                 &  \\
$\thL_m$, $\vL_m$   & posterior mean and variance of client $m$'s personal parameter                             &  \\
$\thFL_m$, $\vFL_m$ & posterior mean and variance of client $m$'s personal parameter conditional on all the data &  \\
$\thG$, $\vG$       & global model's posterior mean and variance                                                 &  \\
$\eta$              & local learning rate                                                                        &  \\
$\ell$              & local learning steps                                                                       &  \\
$t$                 & FL round                                                                                   &  \\
$\th_{m}^{t}$       & client $m$'s FL optimal parameter                                                          &  \\
$\th_{m, t}$        & client $m$'s local optimal parameter                                                       &  \\ \cline{3-3} 
$\th^t$             & global optimal parameter                                                                   &  \\ \hline
\end{tabular}
\end{table*}



\section{An alternative version of Algorithm~\ref{algo} with larger complexity}

% TODO
In Algorithm~\ref{algo_ablation_complex_version}, we summarize a more complicated version of Algorithm~\ref{algo}, which asks each client to run additional local training until convergence (denoted by $\th_{m,t}$), in each FL round. We also report ablation studies. The results (TBD) show that there are only slight gains compared with Algorithm~\ref{algo}. %, which is in line with our convergence analysis.  


%%%%    Algorithm       %%%%%%% 
\begin{algorithm*}[tb]
\SetAlgoLined
\DontPrintSemicolon
\caption{Self-Aware Personal Federated Learning by Introducing Local Minimum ${\color{blue} \th_{m,t}}$ (Augmented Self-FL)}
\label{algo_ablation_complex_version}
\Input{A server and $M$ clients. System-wide objects, including the initial model parameters $\th_{m}^{0} = \th_{m, 0} = \th^0$, initial uncertainty of clients' parameters $\widehat{\vT}=0$, the activity rate $C$, the number of communication rounds $T$, server batch size $B_s$, and client batch size $B_m$, and the loss function $(z, \th) \mapsto \loss(z, \th)$ corresponding to a common model architecture. Each client $m$'s local resources, including the data $z_{m,1}, \ldots, z_{m,N_m}$, parameter $\th_m$, the number of local training steps $\ell_m$, and the learning rate $\eta_m$. 
}
\kwSystem{}{
    \For{\textup{each communication round }$t = 1,2,\dots T$}{

        $\mathbb{M}_t \leftarrow \max(\lfloor C \cdot M \rfloor ,1)$ active clients uniformly sampled without replacement
    
        \For{\textup{each client }$m \in \mathbb{M}_t$\textup{ \textbf{in parallel}}}{
    
            Distribute server model parameters $\th^{t-1}$ to local client $m$
    
            $(\th_{m}^{t}, {\color{blue} \th_{m,t}}, \widehat{\vD_m}) \leftarrow$ \textbf{ClientUpdate}$(z_{m,1},\ldots,z_{m,N_m}, \th^{t-1}, \widehat{\vT})$
        }
        
        $(\th^t, \widehat{\vT}) \leftarrow$ \textbf{ServerUpdate}$(\th_{m}^{t}, {\color{blue} \th_{m,t}}, \widehat{\vD_m}, m \in \mathbb{M}_t)$
    }
}
\kwClient{\textup{$(z_{m,1},\ldots,z_{m,N_m}, \th^{t-1}, \widehat{\vT})$}}{

    Calculate the uncertainty of the local optimal solution $\thL_m$ of client $m$:
    \begin{align}
     \widehat{\vD_m} = \textrm{empirical variance of }\{\th_{m,1}, \ldots , \th_{m,t-1} \} .
    \end{align}
    
    Calculate the initial parameter 
    \begin{align}
    \th_{m}^{t} &\de \th^{t-1} -  \frac{(\widehat{\vT} + \widehat{\vD_m})^{-1} }{\sum_{k \neq m} (\widehat{\vT} + \widehat{\vD_k})^{-1}} (\th_{m, t-1} - \th^{t-1}) ,
    \end{align}

    Choose $\ell_m \geq 1$ according to 
    \begin{align}
    \biggl(1-\frac{\eta_m }{B_m \widehat{\vD_m}} \biggr)^{\ell_m}
    &=  \frac{ \sum_{k\neq m} (\widehat{\vT} + \widehat{\vD_k})^{-1}}{ 1/\widehat{\vD_m} + \sum_{k\neq m} (\widehat{\vT} + \widehat{\vD_k})^{-1} } 
    \end{align}
    
    
    \For{\textup{local step $s$ from $1$ to $\ell_m$}}{
    
        Sample a batch $I \subset [N_m]$ of size $B_m$
        
        Update $\th_{m}^{t} \leftarrow \th_{m}^{t} - \eta_m \nabla_{\th} \sum_{i \in I} \loss (\w_{m,i}, \th_{m}^{t}), $
    }
    
    
    Let ${\color{blue} \th_{m,t}} \leftarrow \th_{m}^{t}$.
    
    {\color{blue}
    \For{\textup{local step $s$ from $\ell_m+1$ to $\infty$}}{
    
        Sample a batch $I \subset [N_m]$ of size $B_m$
        
        Update $\th_{m,t} \leftarrow \th_{m,t} - \eta_m \nabla_{\th} \sum_{i \in I} \loss (\w_{m,i}, \th_{m,t}), $
        
        If {it converges}, then Break.
    }
    
    
    Store ${\color{blue} \th_{m,t}}$ locally
    
    } %color end
    
    Return $(\th_{m}^{t}, {\color{blue} \th_{m,t}}, \widehat{\vD_m})$ and send them to the server
}
\kwServer{\textup{$(\th_{m}^{t}, {\color{blue} \th_{m,t}}, \widehat{\vD_m}, m \in \mathbb{M}_t)$}}{
    Calculate the uncertainty of clients' underlying parameters
    \begin{align}
        \widehat{\vT} = \textrm{empirical variance of }\{{\color{blue} \th_{m,t}}, m \in \mathbb{M}_t\} .
    \end{align}
        
    Calculate model parameters
        \begin{align}
            \th^t &\de \frac{\sum_{m \in \mathbb{M}_t} (\widehat{\vT} + \widehat{\vD_m})^{-1} {\color{blue} \th_{m,t}}}{ \sum_{m \in \mathbb{M}_t} (\widehat{\vT} + \widehat{\vD_m})^{-1} } .
        \end{align}
    
    Return $(\th^t, \widehat{\vT})$
}
\end{algorithm*}
